DeeperCut: A Deeper, Stronger, and Faster Multi-Person Pose Estimation Model

The goal of this paper is to advance the state-of-the-art of articulated pose estimation in scenes with multiple people. To that end we contribute on three fronts. We propose (1) improved body part detectors that generate effective bottom-up proposals for body parts; (2) novel image-conditioned pairwise terms that allow to assemble the proposals into a variable number of consistent body part configurations; and (3) an incremental optimization strategy that explores the search space more efficiently thus leading both to better performance and significant speed-up factors. Evaluation is done on two single-person and two multi-person pose estimation benchmarks. The proposed approach significantly outperforms best known multi-person pose estimation results while demonstrating competitive performance on the task of single person pose estimation. Models and code available at http://pose.mpi-inf.mpg.de

==> section_experiments.tex <==
\section{Evaluation on Multi-Person Pose Estimation}
\label{sec:experiments}
\myparagraph{Datasets and evaluation measures.} MPII Multi-Person:
validation set of randomly sampled $200$ images with X people to
evaluate the parameters; easy subset of 288 images for direct
comparison to~\cite{pishchulin15arxiv}; full set; mAP evaluation
measure. WAF dataset: $m$PCK evaluation measure.
%\input{table_multicut_mpii_multi_subset_462}
\subsection{Results on MPII Multi-Person Dataset}
\input{table_multicut_mpii_multi_subset_200_hierarch}
\input{table_multicut_mpii_multi}
%\input{table_multicut_mpii_multi}
\subsection{Results on WAF Dataset}
\input{table_multicut_waf}



==> table_multicut_mpii_multi.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l c ccc ccc c|c@{}}
    \toprule
    Setting& Head   & Sho  & Elb & Wri & Hip & Knee & Ank & AP & time [s/frame]\\
    \midrule
    \multicolumn{10}{c}{subset of 288 images as in~\cite{pishchulin16cvpr}}\\
    $\deepercut$ (1-stage) & 83.3  & 79.4  & 66.1  & 57.9  & 63.5  & 60.5 & 49.9 & 66.2 & 1333 \\ % exp 787 UBody - 71.7 & 
    $\deepercut$ & \textbf{87.5}  & \textbf{82.8}  & \textbf{70.2}  & \textbf{61.6}  & \textbf{66.0}  & \textbf{60.6} & \textbf{56.5} & \textbf{69.7} & \textbf{230} \\ % exp 786 UBody -  \textbf{75.5} 
    $\deepcut$~\cite{pishchulin16cvpr} & 73.4  & 71.8  & 57.9  & 39.9  & 56.7  & 44.0 & 32.0 & 54.1 & 57995\\ % UBody -  60.7 &
    \midrule
    \multicolumn{10}{c}{full set}\\
    $\deepercut$ (1-stage) & 73.7  & 65.4  & 54.9  & 45.2  & 52.3  & 47.8 & 40.7 & 54.7 & 2785 \\ % exp 794 % UBody - 59.8 & 
    $\deepercut$                & \textbf{79.1}  & \textbf{72.2}  & \textbf{59.7}  & \textbf{50.0}  & \textbf{56.0}  & \textbf{51.0} & \textbf{44.6} & \textbf{59.4} & 485 \\ % exp 790 UBody -  \textbf{65.3} &
    Faster R-CNN~\cite{ren2015faster} + unary &64.9  & 62.9  & 53.4  &
           44.1  & 50.7  & 43.1 & 35.2 & 51.0 & \textbf{1}\\ % UBody - 56.3 & 
    %$\deepcut$~\cite{pishchulin15arxiv} \highp\\
    %\quad + regression pairwise  & 79.9 & 70.4 & 58.9 & 48.1 & 55.0 & 48.3 & 43.1 & 64.3 & 58.1 \\
    %\quad \quad + ResNet      & 77.9 & 72.0 & 59.4 & 51.7 & 56.1 & 53.2 & 48.3 & 65.3 & 60.2 \\
    %\quad \quad \quad + location refinement NMS ($\deepcutplus$) & 78.1 & 72.8 & 61.0 & 53.5 & 57.9 & 55.0 & 49.4 & 66.4 & 61.4 \\
    \bottomrule
  \end{tabular}
  \vspace{0.1em}
\caption[]{Pose estimation results (AP) on MPII Multi-Person.}
\label{tab:multicut:mpii-multi}
\vspace{-0.5cm}
\end{table}


==> table_multicut_mpii_multi_subset_200.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l c ccc ccc cc@{}}
    \toprule
    Setting& Head   & Sho  & Elb & Wri & Hip & Knee & Ank & UBody & FBody \\
    \midrule
    regression pairwise  \highp \\
    \quad + one direction only \highp \\
    \quad + no angle \highp \\
    \midrule
    \quad + ResNet \highp \\
    \quad + location refinement NMS ($\deepcutplus$) \highp\\
    \midrule
    \quad\quad + $\deepcutplush$ \highp \\

    \bottomrule
  \end{tabular}
  \vspace{0.1em}
\caption[]{Pose estimation results (AP) on a validation set of $200$ images from MPII Multi-Person.}
\label{tab:multicut:mpii-multi}
\end{table}


==> table_multicut_mpii_multi_subset_200_hierarch_val.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l c ccc ccc cc|c@{}}
    \toprule
    Setting& Head   & Sho  & Elb & Wri & Hip & Knee & Ank & UBody & FBody & time (s)\\
    \midrule
    1-stage optimize, 100 det, nms 1x & 87.6  & 83.1  & 72.5  & 63.9  & 68.6  & 62.7 & 51.4 & 76.8 & 70.4 & 365 \\ % exp 816
    1-stage optimize, 100 det, nms 2x & 87.2  & 83.2  & 73.8  & 63.3  & 69.6  & 62.0 & 52.3 & 76.9 & 70.6 & 384 \\ % exp 823
    1-stage optimize, 150 det, nms 2x & 88.4  & 84.6  & 73.4  & 64.2  & 70.4  & 63.5 & 50.8 & 77.6 & 71.2 & 784 \\ % exp 769
    \midrule
    2-stage optimize & 92.0  & 86.9  & 77.2  & 67.9  & 70.6  & 64.1 & 55.0 & 81.0 & 73.9 & \textbf{127} \\ % exp 825
    3-stage optimize & 91.0  & 86.0  & 77.3  & 68.7  & 70.5  & 64.0 & 54.5 & 80.8 & 73.7 & 133 \\ % exp 826
    \quad + split detections & \textbf{92.0} & \textbf{88.1}  & \textbf{78.1}  & \textbf{69.7}  & \textbf{71.7}  & \textbf{65.1} & \textbf{55.0} & \textbf{82.0} & \textbf{74.8} & 148 \\ % exp 827
    %\quad\quad + different score threshold \lowp\\
    
    \midrule
    $\deepcut$~\cite{pishchulin16cvpr}
& 55.4  & 48.2  & 40.1  & 30.0  & 38.9  & 27.6 & 19.4 & 43.4 & 37.5 & 30000\\
    \bottomrule
  \end{tabular}
  \vspace{0.1em}
\caption[]{Performance (AP) of different  hierarchical versions of $\deepercut$ on MPII Multi-Person Val.}
\label{tab:multicut:mpii-multi:hierarchical}
\vspace{-0.65cm}
\end{table}


==> table_multicut_mpii_multi_subset_200_pairwise_ablation_val.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l c ccc ccc cc|c@{}}
    \toprule
    Setting& Head   & Sho  & Elb & Wri & Hip & Knee & Ank & UBody & FBody & time (s)\\
    \midrule
    bi-directional + angle & \textbf{87.6}  & \textbf{83.1}  & \textbf{72.5}  & 63.9  & \textbf{68.6}  & \textbf{62.7} & \textbf{51.4} & \textbf{76.8} & \textbf{70.4} & \textbf{365} \\ % exp 816
    uni-directional + angle & 86.4  & 81.7  & 72.2  & \textbf{64.5}  & 67.5  & 62.0 & 50.3 & 76.2 & 69.7 & 2044 \\ %exp 822
    %tree-connected bi-directional + angle & \highp \\
    bi-directional & 84.2  & 80.6  & 70.2  & 61.6  & 67.0  & 62.4 & 51.2 & 74.2 & 68.6 & 1635 \\ % exp 821
    \bottomrule
  \end{tabular}
  \vspace{0.1em}
\caption[]{Effects of different versions of the pairwise terms on the pose estimation performance (AP) on MPII Multi-Person Val.}
\label{tab:multicut:mpii-multi:pairwise:ablation}
\vspace{-0.5cm}
\end{table}


==> table_multicut_mpii_multi_subset_200_pairwise_val.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l l c ccc ccc cc|c@{}}
    \toprule
    Unary\hspace{1.5cm} & Pairwise & Head   & Sho  & Elb & Wri & Hip & Knee & Ank & UBody & FBody & time (s) \\
    \midrule
    $\deepcut$~\cite{pishchulin16cvpr} & $\deepcut$~\cite{pishchulin16cvpr}
    & 55.4  & 48.2  & 40.1  & 30.0  & 38.9  & 27.6 & 19.4 & 43.4 & 37.5 & 30000\\ % expidx 819/829  
    $\deepcut$~\cite{pishchulin16cvpr} & this work & 83.1  & 76.4  & 62.6  & 53.9  & 60.3  & 51.3 & 41.3 & 69.0 & 61.8 & 1779 \\ % expidx 818
    this work & this work & 86.4  & 80.9  & 70.9  & 62.4  & 66.6  & 60.3 & \textbf{53.3} & 75.1 & 69.1 & 770 \\ % expidx 817
    \multicolumn{2}{l}{\quad + location refinement before NMS} & \textbf{87.6}  & \textbf{83.1}  & \textbf{72.5}  & \textbf{63.9}  & \textbf{68.6}  & \textbf{62.7} & 51.4 & \textbf{76.8} & \textbf{70.4} & \textbf{365} \\ % expidx 816
    \bottomrule
  \end{tabular}
  % exp ids: 784 782 780 778
  \vspace{0.1em}
\caption[]{Effects of proposed pairwise and unaries on the pose estimation performance (AP) on MPII Multi-Person Val.}
\label{tab:multicut:mpii-multi:pairwise}
\end{table}


==> table_multicut_mpii_multi_subset_288.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l c ccc ccc cc@{}}
    \toprule
    Setting& Head   & Sho  & Elb & Wri & Hip & Knee & Ank & UBody & FBody \\
    \midrule
    \multicolumn{10}{c}{``easy'' subset of 288 images as in~\cite{pishchulin15arxiv}}\\
    $\deepcutplus$ 83.3  & 79.4  & 66.1  & 57.9  & 63.5  & 60.5 & 49.9 & 71.7 & 66.2 \\
    $\deepcutplush$ 87.5  & 82.8  & 70.2  & 61.6  & 66.0  & 60.6 & 56.5 & 75.5 & 69.7 \highp\\
    $\deepcut$~\cite{pishchulin15arxiv} & 77.2  & 71.8  & 55.9  & 42.1  & 53.8  & 39.9 & 27.4 & 61.8 & 53.2 \\
    \midrule
    \multicolumn{10}{c}{full set}\\
    $\deepcutplus$ \highp\\
    $\deepcutplush$ \highp\\
    $\deepcut$~\cite{pishchulin15arxiv} \highp\\
    %\quad + regression pairwise  & 79.9 & 70.4 & 58.9 & 48.1 & 55.0 & 48.3 & 43.1 & 64.3 & 58.1 \\
    %\quad \quad + ResNet      & 77.9 & 72.0 & 59.4 & 51.7 & 56.1 & 53.2 & 48.3 & 65.3 & 60.2 \\
    %\quad \quad \quad + location refinement NMS ($\deepcutplus$) & 78.1 & 72.8 & 61.0 & 53.5 & 57.9 & 55.0 & 49.4 & 66.4 & 61.4 \\
    \bottomrule
  \end{tabular}
  \vspace{0.1em}
\caption[]{Pose estimation results (AP) on MPII Multi-Person.}
\label{tab:multicut:mpii-multi}
\end{table}


==> table_multicut_mpii_multi_subset_462.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l c ccc ccc cc@{}}
    \toprule
    Setting& Head   & Sho  & Elb & Wri & Hip & Knee & Ank & UBody & FBody \\
    \midrule
    $\deepcut$~\cite{pishchulin15arxiv} \todo{include new solver} & 69.4 & 64.3 & 50.1 & 35.0 & 50.6 & 40.1 & 26.5 & 54.7 & 48.4 \\
    \quad + regression pairwise  & 79.9 & 70.4 & 58.9 & 48.1 & 55.0 & 48.3 & 43.1 & 64.3 & 58.1 \\
    \quad \quad + ResNet      & 77.9 & 72.0 & 59.4 & 51.7 & 56.1 & 53.2 & 48.3 & 65.3 & 60.2 \\
    \quad \quad \quad + location refinement NMS ($\deepcutplus$) & 78.1 & 72.8 & 61.0 & 53.5 & 57.9 & 55.0 & 49.4 & 66.4 & 61.4 \\
    \bottomrule
  \end{tabular}
  \vspace{0.1em}
\caption[]{Pose estimation results (AP) on a subset of images from MPII Multi-Person. 
           For the fair comparison we report the results on the same
           subset of $462$ images, as reported
           by~\cite{pishchulin15arxiv}}
\label{tab:multicut:mpii-multi}
\end{table}

